Polaronic mass renormalization of impurities in BEC: correlated Gaussian wavefunction approach

We propose a class of variational Gaussian wavefunctions to describe Fr\"ohlich polarons at finite momenta. Our wavefunctions give polaron energies that are in excellent agreement with the existing Monte Carlo results for a broad range of interactions. We calculate the effective mass of polarons and find smooth crossover between weak and intermediate impurity-bosons coupling. Effective masses that we obtain are considerably larger than those predicted by the mean-field method. A novel prediction based on our variational wavefunctions is a special pattern of correlations between host atoms that can be measured in time-of-flight experiments. We discuss atomic mixtures in systems of ultracold atoms in which our results can be tested with current experimental technology.

==> commands.tex <==
\global\long\def\ket#1{\left| #1\right\rangle }
 \global\long\def\bra#1{\left\langle #1 \right|}
 \global\long\def\kket#1{\left\Vert #1\right\rangle }
 \global\long\def\bbra#1{\left\langle #1\right\Vert }
 \global\long\def\braket#1#2{\left\langle #1\right. \left| #2 \right\rangle }
 \global\long\def\bbrakket#1#2{\left\langle #1\right. \left\Vert #2\right\rangle }
 \global\long\def\av#1{\left\langle #1 \right\rangle }
 \global\long\def\tr{\text{tr}}
 \global\long\def\Tr{\text{Tr}}
 \global\long\def\pd{\partial}
 \global\long\def\im{\text{Im}}
 \global\long\def\re{\text{Re}}
 \global\long\def\sgn{\text{sgn}}
 \global\long\def\Det{\text{Det}}
 \global\long\def\abs#1{\left|#1\right|}
 \global\long\def\u{\uparrow}
 \global\long\def\d{\downarrow}
  \global\long\def\v#1{\vec{#1}}
 \global\long\def\bs#1{\boldsymbol{#1}}
 \global\long\def\perm#1{\mathrm{perm_s} \left(#1\right)}
 \global\long\def\arr#1#2#3#4{\left(\begin{array}{cc} #1 & #2 \\ #3 & #4\\ \end{array}\right)}
 \global\long\def\q#1#2{\frac{\eta_{#1#2}}{\Omega_{#1}+\Omega_{#2}}}
  \global\long\def\qq#1#2{\frac{\eta_{#1}\eta_{#2} B_{#1}B_{#2}}{\Omega_{#1}+\Omega_{#2}}}
    \global\long\def\qqq#1#2{\frac{\eta_{#1}\eta_{#2} }{\Omega_{#1}+\Omega_{#2}}}
  \global\long\def\qc#1#2{\frac{\eta_{#1#2}^*}{\left( \Omega_{#1}+\Omega_{#2}\right)}}
  \global\long\def\sc#1#2{\vec{#1} \vec{#2}}
\global\long\def\th{\theta}
\global\long\def\mI{\mathcal{M}^{-1}}
\global\long\def\tens#1{\boldsymbol{#1}}



\renewcommand{\l}{\left(}
\newcommand{\llb}{\left\langle}
\renewcommand{\r}{\right)}
\newcommand{\rr}{\right\rangle}
\newcommand{\rf}{\text{rf}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\Ys}{\prod_{j<k}(z_j-z_k)}
\newcommand{\CF}[1]{\hspace{-0.12cm}~^{#1}\text{CF}}
\newcommand{\CB}[1]{\hspace{-0.12cm}~^{#1}\text{CB}}
\newcommand{\CP}[1]{\hspace{-0.12cm}~^{#1}\text{CP}}
\newcommand{\gs}{\text{gs}}
\newcommand{\LLL}{\text{LLL}}
\newcommand{\LN}{\text{LN}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\bkt}[2]{\left\langle #1 |#2 \right\rangle}
\renewcommand{\H}{\hat{\mathcal{H}}}
\renewcommand{\c}{\hat{c}}

\newcommand{\n}{\hat{n}}
\newcommand{\cd}{\hat{c}^\dagger}

\newcommand{\bd}{\hat{b}^\dagger}
\renewcommand{\b}{\hat{b}}
\newcommand{\dd}{\hat{d}^\dagger}
\renewcommand{\d}{\hat{d}}
\newcommand{\bt}{\hat{\beta}}
\newcommand{\btd}{\hat{\beta}^\dagger}

\renewcommand{\a}{\hat{b}}
\newcommand{\ad}{\hat{b}^\dagger}

\newcommand{\lb}{\hat{l}}
\newcommand{\lbd}{\hat{l}^\dagger}
\newcommand{\rh}{\hat{\rho}}
\newcommand{\g}{\hat{\gamma}}
\newcommand{\gd}{\hat{\gamma}^\dagger}
\newcommand{\G}{\hat{\Gamma}}
\newcommand{\Gd}{\hat{\Gamma}^\dagger}
\newcommand{\hc}{\text{h.c.}}
\newcommand{\MF}{\text{MF}}
\newcommand{\BEC}{\text{BEC}}
\newcommand{\D}[1]{\mathcal{D} [ #1 ]}
\newcommand{\imp}{\text{imp}}
\newcommand{\h}{\mathfrak{h}}
\newcommand{\RG}{\text{RG}}
\newcommand{\psd}{\hat{\psi}^\dagger}
\newcommand{\ps}{\hat{\psi}}
\newcommand{\I}{\text{I}}
\newcommand{\p}{\text{p}}
\newcommand{\f}{\text{f}}
\newcommand{\s}{\text{s}}
\renewcommand{\sf}{\text{sf}}
\renewcommand{\O}{\hat{\mathcal{O}}}
\newcommand{\U}{\hat{U}}
\newcommand{\Ud}{\hat{U}^\dagger}
\newcommand{\F}{\hat{F}}



\newcommand{\KP}{\text{KP}}
\newcommand{\HMF}{\mathscr{H}_{\text{MF}}}

\newcommand{\blankpage}{
\newpage
\thispagestyle{empty}
\mbox{}
\newpage
}

\usepackage{array}


\usepackage{bm}	% bold in math mode
%\renewcommand{\vec}[1]{\bm{#1}}

\newcommand{\ph}{\text{ph}}
\newcommand{\IB}{\text{IB}}
\newcommand{\eff}{\text{eff}}
